Vipera: Towards systematic auditing of generative text-to-image models at scale

Generative text-to-image (T2I) models are known for their risks related such as bias, offense, and misinformation. Current AI auditing methods face challenges in scalability and thoroughness, and it is even more challenging to enable auditors to explore the auditing space in a structural and effective way. Vipera employs multiple visual cues including a scene graph to facilitate image collection sensemaking and inspire auditors to explore and hierarchically organize the auditing criteria. Additionally, it leverages LLM-powered suggestions to facilitate exploration of unexplored auditing directions. An observational user study demonstrates Vipera's effectiveness in helping auditors organize their analyses while engaging with diverse criteria.

==> sections/old/02_related_work.tex <==
\section{Related Work}
\subsection{Auditing generative AI}
Generative AI systems, while enhancing productivity, have sparked increasing societal concerns due to potential harmful behaviors, such as social biases and violence~\cite{algorithm-harms}. Consequently, there is a growing emphasis on detecting and mitigating issues within these systems, prompting developers and professional auditors to evaluate them using benchmarks like SafetyBench~\cite{zhang2023safetybench} and AgentHarm~\cite{andriushchenko2024agentharm}. However, the limited variety of inputs, contexts, and scenarios in these benchmarks poses challenges in adequately assessing real-world performance. Recent research emphasizes the importance of involving general end users in the auditing process, highlighting their ability to uncover overlooked cases and share valuable insights~\cite{everydayaudit,enduseraudits,crowdsourced-failure-reports,deng2025weaudit}. Despite this potential, systematically auditing these systems through crowdsourcing remains difficult and costly, as the data size, auditing criteria, and insights available to individual auditors are often limited. This underscores the need for approaches that enable scalable auditing.

Recent studies have begun to focus on scalable auditing of generative AI, primarily addressing two key challenges. First, evaluating numerous system outputs and helping users comprehend the results within a limited timeframe is difficult. To tackle this, human-in-the-loop auditing has been proposed, utilizing large language models for automatic system evaluation while accommodating user inquiries and organizing results for human interpretation~\cite{llm-as-a-judge, who-validates, llm-audit-llm}. Further efforts have introduced annotations and visualizations to enhance the understanding of auditing results~\cite{gero-atscale, adversaflow}. The second challenge pertains to auditing criteria. Early tools relied on quantitative NLP metrics (e.g., ROUGE) or adhered to a predefined list of criteria, which often proved inflexible and lacking comprehensiveness. Recently, Kim et al. addressed this limitation by allowing users to define their own criteria~\cite{evallm}.

While these approaches effectively audit text-to-text models, extending them to text-to-image models presents challenges. Images contain richer semantic information (e.g., objects and styles) that can lead to a diverse range of auditing criteria, yet there is a notable lack of tools to assist auditors in interpreting auditing results for iterative assessments in the image context. To address this, Vipera integrates visual cues and AI-driven auditing suggestions, facilitating a structured and systematic exploration of auditing criteria. It also includes visualizations that enhance sensemaking and comparison of image sets.

\subsection{Visual analytics for image collection sensemaking}
Sensemaking of large image collections plays a key role in auditing T2I models at scale, and visual analytics approaches have proven effective in this context~\cite{afzal2023visualization}. One common method involves clustering images based on pixel or vector embeddings for visualization, which supports various analytical tasks such as search and exploration, comparison, and visual summarization~\cite{ii20,schmidt2013vaico,pan2019content}. To incorporate image semantics alongside visual features, recent works identify semantic objects within images and extract concise textual representations—such as keywords, descriptions, or captions. These text analysis results facilitate tasks like semantic categorization and pattern mining~\cite{xie2018semantic,yee2003faceted,li2024visual}. However, characterizing the relationships between objects using plain text can be challenging. To address this, scene graphs have emerged as a more expressive representation, where nodes denote semantic objects and edges illustrate their relationships. This representation enhances detailed understanding of image collections and improves analysis performance~\cite{fang2017narrative,johnson2015image}.


With the advent of generative T2I models, a recently emerged task is to visualize the relationship of between prompts and corresponding images. For instance, DreamSheets~\cite{dreamsheets} organizes prompts and images in a spreadsheet layout to facilitate comparison. PrompTHis~\cite{guo2024prompthis} introduces an \textit{image variant graph} to illustrate the semantic transitions of image clusters as users create new prompts. However, these approaches often struggle to support sensemaking in large-scale image sets, where variations among outputs for a single prompt can lead to overly condensed visual clusters. In response, Vipera embeds bar charts within a tree-based scene graph, revealing distributional patterns for images related to individual prompts and allowing for comparisons across prompts. Additionally, it leverages the scene graph as a visual aid to foster systematic and structured AI auditing while providing inspiration to auditors. 

